A well-balanced reconstruction with bounded velocities for the shallow water equations by convex combination

Finite volume schemes for hyperbolic balance laws require a piecewise polynomial reconstruction of the cell averaged values, and a reconstruction is termed `well-balanced' if it is able to simulate steady states at higher order than time evolving states. For the shallow water system this involves reconstructing in surface elevation, to which modifications must be made as the fluid depth becomes small to ensure positivity, and for many reconstruction schemes a modification of the inertial field is also required to ensure the velocities are bounded. We propose here a reconstruction based on a convex combination of surface and depth reconstructions which ensures that the depth increases with the cell average depth. We also discuss how, for cells that are much shallower than their neighbours, reducing the variation in the reconstructed flux yields bounds on the velocities. This approach is generalisable to high order schemes, problems in multiple spacial dimensions, and to more complicated systems of equations. We present reconstructions and associated technical results for three systems, the standard shallow water equations, shallow water in a channel of varying width, and a shallow water model of a particle driven current. Positivity preserving time stepping is also discussed.

==> Templates/StandardMathsMacros.tex <==
%My macros for the math environment

\usepackage{xparse}
\makeatletter




%---BRACKETS----

%Normal brackets

\DeclarePairedDelimiter{\ppar}{\lparen}{\rparen}
\DeclarePairedDelimiter{\pang}{\langle}{\rangle}
\DeclarePairedDelimiter{\pbrc}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\pbrk}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\pgrp}{\lgroup}{\rgroup}

%Bracket-like structures

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\round}{\lfloor}{\rceil}

\DeclarePairedDelimiter{\eval@wdot}{.}{\rvert}
\NewDocumentCommand{\eval}{som}{%
	\IfBooleanTF{#1}
    	{\eval@wdot*{#3}}
   		{\IfNoValueTF{#2}{#3\rvert}{\eval@wdot[#2]{#3}}}%
}

\DeclarePairedDelimiterX{\setpred}[2]{\lbrace}{\rbrace}{\: #1 \: \delimsize\vert \: #2 \:}




%---OPERATORS---

\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\minmod}{minmod}
\DeclareMathOperator{\diag}{diag}




%---DIMENSIONLESS CONSTANTS---
%Define carefully, some of these are defined in the JFM template

%\Rey Reynolds number 
\ifdefined\Rey\else
	\newcommand\Rey{\mbox{\textit{Re}}}
\fi

%\Pran Prandtl number
\ifdefined\Pran\else
	\newcommand\Pran{\mbox{\textit{Pr}}} 
\fi

%\Pen Peclet number
\ifdefined\Pen\else
	\newcommand\Pen{\mbox{\textit{Pe}}}
\fi

%\Fro Froude number
\ifdefined\Fro\else
	\newcommand\Fro{\mbox{\textit{Fr}}}
\fi

%\Ric Richardson number
\ifdefined\Ric\else
	\newcommand\Ric{\mbox{\textit{Ri}}}
\fi




%---CALCULUS---
%Uses the calculus syntax from the Physics package with a few modifications
%
%For fractions p/q, following applies
%\frac{p}{q}, standard
%\frac*{p}{q}, flat
%\frac**{p}{q}, flat, autosize slash
%\frac*[\size]{p}{q}, flat, slash size of \size
%
%For differential d syntax is
%\dd*[power]{measure}
%Star removes spacing
%
%For derivative df/dx, stars the same as for \frac, optional argument the order of the derivative
%\dv(frac syntax here)[order]{f}{x}
%If wanting to use a flat derivative without sizing with order, then \dv*[][n]{f}{x}
%
%For partial derivative df/dx, use \pdv with syntax as for \dv
%NOT IMPLEMENTED YET Alternatively, for d^n f/dx_1 ... dx_n use
%\pdvm(frac syntax here){n}{f}{x_1}...{x_n}

%\frac
\let\frac@nostar\frac
\DeclarePairedDelimiterX{\frac@starwdot}[2]{.}{.}{#1 \delimsize/ #2}
\NewDocumentCommand{\frac@star}{somm}{%
	\IfBooleanTF{#1}
    	{\frac@starwdot*{#3}{#4}}
    	{\IfNoValueTF{#2}{#3/#4}{\frac@starwdot[#2]{#3}{#4}}}%
}
\renewcommand*\frac{\@ifstar{\frac@star}{\frac@nostar}}

%\dd
\NewDocumentCommand{\dd}{som}{%
	\IfBooleanF{#1}{\,}%
	\IfNoValueTF{#2}{%Check whether optional argument is given
		\textrm{d} #3%
	}{%
		\textrm{d}^{#2} #3%
	}%
	\IfBooleanF{#1}{\,}%
}

%\dv
\NewDocumentCommand\dv@nostar{O{}mm}{%
	\frac@nostar{\textrm{d}^{#1} #2}{{\textrm{d} #3}^{#1}}
}
\NewDocumentCommand{\dv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\textrm{d}^{#2} #4}{{\textrm{d} #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\textrm{d}^{#3} #4}{{\textrm{d} #5}^{#3}}%
		\else
			\frac*[#2]{\textrm{d}^{#3} #4}{{\textrm{d} #5}^{#3}}%
		\fi
	}%
}
\newcommand*\dv{\@ifstar{\dv@star}{\dv@nostar}}

%\pdv
\NewDocumentCommand\pdv@nostar{O{}mm}{%
	\frac@nostar{\partial^{#1} #2}{{\partial #3}^{#1}}
}
\NewDocumentCommand{\pdv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^{#2} #4}{{\partial #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\else
			\frac*[#2]{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\fi
	}%
}
\newcommand*\pdv{\@ifstar{\pdv@star}{\pdv@nostar}}

%%\pdvm
%\NewDocumentCommand\pdvm@nostar@two{mmmm}{%
%	\frac{\partial^2 #2}{\partial #3 \partial #4}
%}
%\NewDocumentCommand{\pdvm@star@two}{sO{}mmm}{%
%	|#1,#2,#3,#4,#5|
%%	\IfBooleanTF{#2}{%
%%		\frac**{\partial^2 #4}{\partial #5 \partial #6}%
%%	}{%
%%		\if \relax\detokenize{#3}\relax
%%			\frac*{\partial^2 #4}{\partial #5 \partial #6}%
%%		\else
%%			\frac*[#3]{\partial^2 #4}{\partial #5 \partial #6}%
%%		\fi
%%	}%
%}
%\newcommand*\pdvm@nostar[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm@STAR[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm{\@ifstar{\pdvm@star}{\pdvm@nostar}}

%\def\pdvm@str@frac{frac}
%\def\pdvm@str@flat{flat}
%\def\pdvm@str@slsh{slsh}
%
%\NewDocumentCommand{\pdvm@two}{mmmmm}{
%	F|#1,#2,#3,#4,#5|
%}
%
%\newcommand*\pdvm@nostar[1]{%
%	A|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@frac}{}%
%	\fi%
%}
%\newcommand*\pdvm@star[2]{%
%	B%\abs{ #1 , #2 } \:
%%	\ifnum #2=2
%%		\pdvm@two{\pdvm@str@slsh}{#1}%
%%	\fi%
%}
%\newcommand*\pdvm@sstar[1]{%
%	C|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@flat}{}%
%	\fi%
%}
%
%\newcommand\pdvm@staropt[1][]{%
%	a| #1 | \:%
%	\if \relax\detokenize{#1}\relax
%		b%
%		\pdvm@star{}%
%	\else
%		c%
%		\pdvm@star{#1}%
%	\fi
%}
%\newcommand*\pdvm@STAR{\@ifstar{\pdvm@sstar}{\pdvm@staropt}}
%\newcommand*\pdvm{\@ifstar{\pdvm@STAR}{\pdvm@nostar}}


%---ORDER NOTATION---

%If order is used with an empty argument then dont use parenthesis
\newcommand{\order@text}[1]{	
	\if\relax\detokenize{#1}\relax% #1 is empty
	\else% #1 is nonempty
		\ppar*{#1}%\qty(#1)
	\fi
}

%Big O
\newcommand{\order}[1]{
	\mathcal{O}\order@text{#1}
}

%Little O
\newcommand{\lorder}[1]{
  	\mathchoice
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \displaystyle
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \textstyle
    	{{\scriptscriptstyle\mathcal{O}}\order@text{#1}}% \scriptstyle
    	{\scalebox{.6}{${\scriptscriptstyle\mathcal{O}}\order@text{#1}$}}%\scriptscriptstyle
  	}

%Big Theta
\newcommand{\Torder}[1]{
	\mathit{\Theta}\order@text{#1}
}




%---ASSORTED---

%Have equation span full width of collumn (good for equations in lists)
\newcommand{\eqnwide}{\displayindent0pt \displaywidth\textwidth}

%Use as 10^\nth
\newcommand{\nth}{\text{th}}

%Defined to be equal to
\newcommand{\eqdef}{\vcentcolon =}%{\stackrel{\mathrm{def}}{=}}

%Text style fraction
\newcommand{\textfrac}[2] {{\textstyle\frac{#1}{#2}}}

%Omitted dummy variable as a dot
\newcommand*\omitdummy{\mathchoice
	{\omitdummy@{\displaystyle}{0.6}}
	{\omitdummy@{\textstyle}{0.6}}
	{\omitdummy@{\scriptstyle}{0.7}}
	{\omitdummy@{\scriptscriptstyle}{0.8}}
}
\newcommand*\omitdummy@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}




%---ENVIRONMENTS---

%Like cases but with as many collumns as you like

\newenvironment{multicasesnobrac}[1][1]{%
%No braces
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}
}
\newenvironment{multicases}[1][1]{%
%Left braced
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}\right.
}
\newenvironment{multicasesd}[1][1]{%
%Left braced with display style
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{>{\displaystyle}{r}@{}>{\displaystyle}{l}}}
}{
	\end{array}\right.
}




%---SIDE BY SIDE SUBEQUATIONS---

%Multiple labeled equations on same line
\newlength{\sbsse@Wl}	%Width of left equation
\newlength{\sbsse@Wm}	%Width of mid text
\newlength{\sbsse@Wr}	%Width of right equation
\newlength{\sbsse@Wt}	%Width of tag
\newlength{\sbsse@We}	%Remaining width on line
\newlength{\sbsse@Wd}	%Remaining width divided into pieces

%Two equations side by side
\newcommand\sidebysidesubequations[6]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    midtext
	% #5    right subequation
	% #6    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{\text{#4}}
	\def\sbsse@Er{#5}
	\def\sbsse@Et{(\ref*{#1}a,b)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space, and midtext if any
			\if\relax\detokenize{#4}\relax
				\setlength{\sbsse@Wd}{\sbsse@We/3}
				\hspace{\sbsse@Wd}
			\else
				\setlength{\sbsse@Wd}{\sbsse@We/4}
				\hspace{\sbsse@Wd}\sbsse@Em\hspace{\sbsse@Wd}
			\fi
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#6}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}

%Three equations side by side
\newcommand\sidebysidesubequationsT[7]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    mid subequation
	% #5	mid label
	% #6    right subequation
	% #7    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{#4}
	\def\sbsse@Er{#6}
	\def\sbsse@Et{(\ref*{#1}a,b,c)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	\setlength{\sbsse@Wd}{\sbsse@We/4}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space
			\hspace{\sbsse@Wd}
			%Mid equation and label
			\sbsse@Em\refstepcounter{equation}\ltx@label{{#5}}
			%Space
			\hspace{\sbsse@Wd}
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#7}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}




\makeatother
